Explainable Artificial Intelligence for Quantifying Interfering and High-Risk Behaviors in Autism Spectrum Disorder in a Real-World Classroom Environment Using Privacy-Preserving Video Analysis

Rapid identification and accurate documentation of interfering and high-risk behaviors in ASD, such as aggression, self-injury, disruption, and restricted repetitive behaviors, are important in daily classroom environments for tracking intervention effectiveness and allocating appropriate resources to manage care needs. However, having a staff dedicated solely to observing is costly and uncommon in most educational settings. Recently, multiple research studies have explored developing automated, continuous, and objective tools using machine learning models to quantify behaviors in ASD. However, the majority of the work was conducted under a controlled environment and has not been validated for real-world conditions. In this work, we demonstrate that the latest advances in video-based group activity recognition techniques can quantify behaviors in ASD in real-world activities in classroom environments while preserving privacy. Our explainable model could detect the episode of problem behaviors with a 77% F1-score and capture distinctive behavior features in different types of behaviors in ASD. To the best of our knowledge, this is the first work that shows the promise of objectively quantifying behaviors in ASD in a real-world environment, which is an important step toward the development of a practical tool that can ease the burden of data collection for classroom staff.

==> figures/fold-subjects.tex <==
\begin{figure}[H]
    \centering
    \includegraphics[width=0.5\linewidth]{figures/fold-subjects.jpg}
    \caption{\small Distribution of subjects across folds in 5-fold cross-validation run on Camera 2. Note how there is minimal data on \textit{S07} and \textit{S09} beyond fold 0, meaning that when testing on this fold, the model has difficulties modeling the behavior of participants for whom it did not have enough training examples. This leads to a lower classification accuracy on this fold.
    \hyeok{What is the point of showing analysis on camera 2, which performance was near random chance? I would discuss only on camera 1.
    And, remove this figure and replace with personalization test result where X-axis is the portion of subjects from test set included in training set and Y-axis is the F1 score from camera 1.}
    }
    \label{fig:fold-subjects}
\end{figure}

==> sections/old_version/intro_2024.02.15.tex <==
\section*{Introduction}

% This template should be used as a starting point for AMIA submissions.  A number of Word styles, all beginning with the word ``AMIA", are available for use in your submissions.

% It is important to review the AMIA Call for Participation where types of submissions considered and general requirements for each submission type are listed. All submissions must conform to the format and presentation requirements described in the CFP and at the submission site.
Autism Spectrum Disorder (ASD) is a neurodevelopmental disorder that manifests itself through a diverse range of behaviors \hyeok{citation}.
Common symptoms include difficulties in understanding and interpreting social cues, challenges in verbal and nonverbal communication, and repetitive behaviors or restricted interests \hyeok{citation}.
While the exact cause remains elusive, a combination of genetic and environmental factors is believed to contribute to the development of ASD.
\hyeok{Make sure you include citations where information is sourced from. Also, this paragraph is too short. Merge with the one below.}

The current diagnostic process relies on clinical observations, developmental history, and standardized assessments \hyeok{What are the standardized assessments provide some examples briefly}, with ASD being typically detected early in childhood.
Visual observation and analysis of children’s natural behaviors are key to detecting
developmental disorders such as ASD. 
While a gold standard observational tool is available, there are limitations hindering a more objective, scalable, and efficient means of detecting and understanding autism.
Observations by a clinician are often subjective and inconsistent \cite{taylor2017} and behavioral ratings are usually not captured in natural environments. 
Moreover, access to trained neurologists and mental health experts is a challenge for most. 
Only 25\% of the world's population had access to more than one neurologist per 100,000 people. In the United States itself, twenty states classify as neurology deserts \cite{rao2017neurodesert}, having less than 10 neurologists per 10000 cases per year. 
\hyeok{How is the accessibility issue relevant to this paper? Try to avoid including irrelevant information in a paper. This paper is more about objectively quantifying activity phenotypes and automated and continuous detection of problem behavior in Autism. Also, is the neurologist fit here? it should be a combination of psychologists, pediatricians, and neurologists. Maybe we can say, developmental disorder specialists? or just say, clinicians? Please check with CFD team.}
Hence, technological solutions ensuring reliable, consistent \hyeok{Have you discussed anything related to inconsistency in assessments, such as interrater reliability? And, also if you would provide how low the interrater reliability is based on citations}, and accurate \hyeok{Accurate can mean anything. Change it to objective} 
identification of ASD is critical. This is especially true given the rising rates of ASD in the global population \cite{zeidan2023autism}.
\hyeok{I think this paragraph is misleading about the major contribution of your work. Our work is not about distinguishing Autism and Healthy kids. This is about a system that can objectively detect and explain problem behaviors in autism. Cut down your text regarding Autism vs. health and refocus it on our major contribution. Get to the point as soon as possible.}

Computer vision has been among the forefront of technological innovations in detecting ASD.
\hyeok{We are not detecting ASD. Our subjects are already diagnosed with Autism and the goal is to objectively detect problem behaviors in Autism.
First start with overall approaches explored in quantifying (or detecting) problem behavior in ASD. What kind of techniques were used? What were there findings overall? But, what are there limitations? Make sure you include citations!}
Different kinds of information have been captured and analyzed with the aid of computer vision such as magnetic resonance imaging (MRI) and functional magnetic resonance imaging (fMRI) data, eye gaze, facial expressions and motions, motor control and movement patterns, stereotyped behaviors, as well as multimodal data. \cite{de2020computer}. \hyeok{This text looks irrelevant as the thesis statement in this paragraph is irrelevant. Also, I think the method is a secondary importance in this work. The primary contribution is the analysis of the dataset containing real-world classroom activities.}

However, technological progress involving machine learning solutions in this field has yet to gain wide acceptance. \hyeok{Are you sure? Thomas also has papers even before I started PhD about aggressive behavior detection in Autism. It has been explored from a while ago. Have you checked a sufficient number of review or survey papers? What is the citation for this claim?}
Controlled settings in clinical environments \hyeok{Is it controlled environment or clinical environment? These two have different notions.} also make the quantification and observation of natural behaviors difficult, which is one of the biggest challenges in using computer vision for autism analysis. \hyeok{This sentence does not make sense. Why is a controlled environment more challenging for using computer vision for ASD analysis? This is not true. And also, the problem of controlled study is that it does not capture activities in a naturalistic environment nothing related to computer vision.}
Moreover, it is also imperative to recognize the diverse presentation of ASD, as individuals may exhibit a wide range of abilities and challenges.
There are often significant variations based on population, age, gender, race, ethnicity, etc. \hyeok{Need citations! Also do we have subject with varying demographics? If not, I think you are inviting for critics. Also, our study is not really about diversity of ASD. Try avoid including unnecessary texts.}
As a result, models trained on curated training data often fail to replicate results on real-world datasets, making them unreliable for clinicians in practice.
\hyeok{Is the focus of our paper on tackling the lack of diversity in ASD dataset in previous work? I don't think so.}
\hyeok{I think this paragraph needs to be rewritten to refocus this work for the dataset challenge. A central contribution of our work is the collection and analysis of ASD behaviors observed in real world classroom and a method to analyze such dataset for scene-level problem behavior detection.
Focus and discuss what the previous dataset looked like. What did it look like? what was the limitations? what is the gap between the existing dataset and the real world? how our work is addressing this gap? Always include citations!}

We address both of these issues \hyeok{What issues? I think they are hidden in text as well as misleading. you need to be more specific and actually mention what issues you are addressing} in our study by teaming up with clinical experts and healthcare professionals at The Center For Discovery (TCFD) \hyeok{This detail is not needed in the introduction. You need to focus on high-level contribution.}. 
Their expert inputs helped us develop an annotated set of problem behaviors to identify ASD. \hyeok{The collaboration with health and engineer is something already expected in this work and no need to emphasize. Furthermore, almost all major previous work are doing that already, which makes this not our major contribution. Don't need to mention it.} 
Moreover, we also utilized TCFD's school facility, featuring a real-world classroom environment for children with autism. \hyeok{You may introduce how classroom activity is conducted in HIGH LEVEL to give an idea how our dataset looks like. Not much detail is needed.}
We helped them set up an expansive camera network, enabling us to continuously monitor these children's behaviors in semi-naturalistic settings. \hyeok{Did we really helped them? I don't think so, although this is our future direction using Raspberry Pi. We are currently using the surveillance camera installed in the facility. And, you can simply mention that you are using these cameras. Also, it is not semi-naturalistic setting. It is actual classroom activity happening in the facility.}
Since autism is often treated by carefully observing behaviors from childhood, we believe that this setup could offer useful insights into ASD in children. \hyeok{What useful insight? Be more scientific and specific! Vague terms should be avoided.}
\hyeok{The introduction is needed to make the reader excited and our audiences are experts in ML, BMI, and ASD (potentially) so you would only focus your text on major scientific contributions. And in this paragraph you would actually want to describe in high level the dataset we collected like which population, What N? and so on with the kind of technique we used, and the major experiment result, assuming that you have sufficiently motivated that this paper is about a new kind of analysis of its kind in ASD behavior detection with the application of explainable AI method.}

Leveraging machine learning and computer vision, we were able to analyze a large scale real-world dataset that would be infeasible for humans.
\hyeok{how large scale? Be more specific! And, you don't have to mention machine learning and computer vision. previous work has also used them. You may want to emphasize the computational efficiency here actually.}
% We hope that such methods that take advantage of the latest machine learning techniques and are developed to perform in the wild will ultimately bridge the gap in access to quality healthcare.
We summarize our contributions as follows:

\begin{itemize}
    \item We study autism behaviors in a real-world classroom setting, which is a unique \hyeok{What do you mean by unique? It can mean anything depend on the context}, heterogeneous environment \hyeok{Are we? I think the video is recorded in a single classroom but with multi-views}, with subjects \hyeok{children with ASD}  exhibiting natural behavior \hyeok{interactions with peers and teachers}. 
    We also did this within a multi-person view, with autistic subjects\hyeok{Never use disease-centric word. Use human-centric work, like children (living) with ASD} as well as neurotypical people \hyeok{Are you sure? Only the teachers? Check with CFD} in the same scene.
    Our participant pool was also evolving with subjects moving between classes, graduating, new students enrolling, etc., causing our model to encounter new participants with time. \hyeok{Too much details}
    The presence of such real-world conditions addresses a significant gap within prior literature, most of which has focused on individual behaviors observed in constrained settings such as clinical environments.
    \hyeok{Be very concise with only 1 to 2 sentences for summarizing contribution. Too many details are mentioned here, which have to be in main paragraph before these bullet lists.}
    
    \item We study autism expressions among school age children. While ASD is often diagnosed before a child attains school-going age, identifying behavioral expressions displayed by school-age children can help us devise models and protocols better suited for such populations. Along this vein, we also analyze and discuss real-world performance considerations when deploying such models. To the best of our knowledge, this is one of few real-time behavior analysis works within ASD which outlines and studies deployment considerations.
    \hyeok{Okay, first, Is studying school-age children with ASD a major contribution of our work? If it is so, you should have discussed this in any previous paragraphs. When you add this discussion, make sure you add citations, as it is difficult to believe that it is the first work that studies this age range of children with ASD. Have you checked a sufficient number of survey articles in behavior analysis in children with ASD? Also, we are not deploying the model, we are developing the model using a dataset captured in a real-world classroom. Also you mention that this is a real-time behavior analysis work. You haven't discussed anything about the computational time of your model. And, it also needs citations where you discuss this, otherwise, it is difficult to believe it is the first real-time behavior analysis work. I think this is a future work as I am not sure if the CFD team has developed data processing pipeline where we can only plug our model for real-time analsys yet. So, it can potentially be a real-time analysis system in the future but not now. Do NOT overclaim your contribution with what not actually is.}

    \item We also dive deeper into the model architecture to analyze what it learns \hyeok{What architecture? Have you discussed this anywhere before? Nothing should come out as a surprise here as you are trying to close the introduction.}. 
    This is achieved using the attention mechanism, which also helps focus the model on the most important features. Analyzing the attention feature maps helped us collect behavioral phenotypes for our study population, which when verified with human experts, prove that our model learns useful signals. This is an important contribution, representing a novel use of attention in the context of interpretability for behavior modeling.
    \hyeok{First of all, have each sentence in separate lines. This helps to jump to the exact sentence location from pdf double-click. Otherwise, I shall search through the paragraph.}
    \hyeok{Make it concise with high-level description about what your explainable model will detect and what you will further analyze. We have discussed multiple time about clustering analysis to find representative behaviors in each activity class. 
    BTW, I haven't seen this yet. Without such extensive analysis in using attention model, there is no point of selling this paper anything related to explainable AI for ASD.}
    
\end{itemize}

\hyeok{Okay. A major structural change is needed in the introduction. Make sure have this flow:
1) What is ASD and what is the healthcare pressure and public burden, economic cost due to this?
2) What kind of behaviors are observed in ASD and why is it important to quantify these clinically? How does it help more targetted and personalized intervention for improving ASD condition?
3) What kind of study has been done previously to quantify problem behavior? And what were their population, study setting, and sensors used? And, what are common limitations they have? What kind of technique they used? Did they use hand-crafted features? If so, can they accurately capture complex and heterogeneous problem behaviors in ASD sufficiently well? If they use deep learning models, have anywork used explainable AI techniques? If so, what are the limitations.
4) What is the major contribution of our work? 1. Study in real world classroom and 2. explainable deep learning model to objectively quantify complex activity phenotypes in movement features and 3) privacy preserving computer vision system.
5) High-level description of our dataset (classroom size, camera viewpoints, size of N, duration of video data, etc)
6) Specific characteristics of our explainable AI model, what are we trying to capture? why automated person attention, temporal attention, and body part attention needed? What makes them necessary to quantify problem behaviors in ASD?
7) How do we keep privacy of the subjects? Why pose-based method is important. Include brief discussion on why using raw frame data can leak identifiable information. There are a lot of work that says that you can retrieve the training data only from hacking the trained model.
8) What were the major experiment (quantitative) results and qualitative results? Again, as I mentioned earlier without actual extensive feature analysis detected by attention model, there is no point of even talking about explainable AI in this paper.
9) What is the broader implication of this work? Why is it a important step toward understanding problem behaviors in ASD? And what are our future work to fill the remaining gap in this direction of research?
10) Lastly, make sure you add all the citations that are necessary!! A lot of your claims here are missing citations.}
    
% The treatment landscape for ASD is multifaceted, encompassing behavioral interventions, speech and language therapy, occupational therapy, and, in some cases, pharmacological interventions. Applied Behavior Analysis (ABA) is a widely utilized behavioral therapy that focuses on reinforcing positive behaviors and reducing undesirable ones. Speech and language therapy aims to enhance communication skills, while occupational therapy addresses sensory and motor challenges. Each treatment plan is tailored to the specific needs of the individual, acknowledging the unique nature of ASD presentations.

% In the context of children with ASD, early intervention is pivotal for fostering optimal development and mitigating the impact of symptoms. Educational support, specialized therapies, and collaboration between parents, educators, and healthcare professionals play a central role in providing comprehensive care for children on the autism spectrum. As our understanding of ASD continues to evolve, ongoing research endeavors seek to unravel the complexities of the disorder, with the ultimate goal of improving diagnostic accuracy, developing targeted interventions, and enhancing the overall well-being of individuals affected by ASD.


==> sections/related_work.tex <==
% \section*{Related Work}
% \barun{merge with intro. After you set everything up, add the related work, and then highlight contributions of this work and how it addresses previous limitations}



% \subsection*{Machine learning in ASD}
% \paragraph{Machine Learning in ASD}
% Several machine learning approaches have been used to study ASD using a variety of algorithms to learn patterns from screening instruments, patient attributes, genetic data, observed behaviors and social interactions.
% \hyeok{why past tense? It is an active research area.}. 
% \resolved
% For instance, Raj \textit{et. al} compared the accuracy in detecting ASD from patient attributes including age, sex, nationality, screening test type and screening test scores \hyeok{from what?} across a variety of models such as support vector machines, convolutional neural networks, Naive Bayes, K-nearest neighbors and logistic regression \cite{raj2020mlasd}. 
% \hyeok{What do you mean with non-clinical datasets? need to be specific. And, I don't think we use this term elsewhere}
% collected from the UCI Machine Learning Repository 
% \hyeok{This detail is not needed. Just adding citation can tell you about where the dataset is archived. Focus on the scientific content of the dataset. And, you have to add citations!!}.
% \resolved
% containing attributes such as age, sex, nationality, screening test type, test scores, etc. 
% Their experiments, conducted on publicly available datasets, found CNN-based classifiers to have the highest accuracy, specificity and sensitivity for detecting autism.  
% \hyeok{Okay. so you referred only a single paper working on ML in ASD as a example with traditional ML use case, but you end this paragraph saying that they are using CNN. This is a conflicting and very shallow discussion.
% What do you mean by traditional ML in the first place? And why CNN is a traditional ML model? I suppose you are meaning shallow models and deep models?}
% \hyeok{The discussion on how ML is used in ASD analysis is needed in this discussion, but you need to discuss more than one. Also what kind of dataset the work you mentioned is using? The context of work is important.}
% \hyeok{The related work is used to highlight the contribution of your work! You have to select sufficient number of work with sufficient level of discussion so that you can emphasize how your model is filling the gap in current state-of-the-arts in ASD behavior analysis with the long-term goal of the research community.}
% \resolved
% Baadel \textit{et. al} recently proposed a clustering approach to identify similar traits in ASD, instead of using a scoring function, as is more common \cite{baadel2020clustering}.
% Their approach, Clustering-based Autistic Trait Classification (CATC) showed a significant improvement in ASD classification, with Random Forests being the best performing classifier.
% They collected data using a mobile screening tool called ASDTests, which contains questionnaires based on a combination of multiple screening methods such as Q-CHAT 10 and AQ-10.
% CATC, when applied to off-the-shelf classification algorithms such as Random Forests, RIPPER \cite{cohen1995ripper} and PART \cite{frank1998part}, improved accuracy, sensitivity and specificity in classifying ASD.

% Algorithms have also been developed focusing on input optimization and feature transformation techniques. Goel \textit{et. al} proposed a Modified Grasshopper Optimization Algorithm (MGOA) \cite{goel2020modified}.
% MGOA with a random forest classifier outperformed other basic ML models, attaining nearly 100\% accuracy, sensitivity and specificity.
% Surest \textit{et. al} proposed a Differential Evaluation (DE) algorithm to find the optimal solution for SVM parameters \cite{suresh2019differential}.
% DE-tuned SVMs were shown to outperform standard SVMs as well as standard and DE-tuned artificial neural networks in ASD classification.

% Computer vision has been among the frontrunners of technological innovations in studying ASD.
% \hyeok{We are not detecting ASD. Our subjects are already diagnosed with Autism and the goal is to objectively detect problem behaviors in Autism.
% First start with overall approaches explored in quantifying (or detecting) problem behavior in ASD. What kind of techniques were used? What were there findings overall? But, what are there limitations? Make sure you include citations!}
% Different kinds of information have been captured and analyzed with the aid of computer vision such as magnetic resonance imaging (MRI) and functional magnetic resonance imaging (fMRI) data, eye gaze, facial expressions and motions, motor control and movement patterns, stereotyped behaviors, as well as multimodal data. \cite{de2020computer}. 
% \hyeok{This text looks irrelevant as the thesis statement in this paragraph is irrelevant. Also, I think the method is a secondary importance in this work. The primary contribution is the analysis of the dataset containing real-world classroom activities.}
% \resolved
% Alkahtani \textit{et. al} \cite{math11194208} studied the effectiveness of LSTM and long-term recurrent neural networks on diagnosing autism by classifying between stimming and normal behaviors from videos. 
% Their experiments showed an impressive 93\% and 96\% accuracy respectively, when evaluated on the publicly available Self-Stimulatory Behavior Dataset.
% However, their work exclusively focused on only one set of behaviors, that were also captured in a clinical setting, and hence not entirely representative of behaviors observed in real-world conditions.

% \hyeok{First of all, let's merge related work in the introduction. 
% Standard biomedical journals do not have separate related work sections. try to integrate these texts smoothly into the introduction section, where it belongs.}

% \paragraph{Behavior analysis and assessment}
% Despite significant ML research into areas such as fMRI analysis, eye gaze tracking and genetic data, behavior analysis has consistently shown highly promising results.
% For instance, Plitt \textit{et. al} demonstrated that behavioral measures were superior to rs-fMRI classifiers for ASD classification \cite{plitt2015functional}.
% Atypical behaviors demonstrated by individuals with ASD are often assessed and during screening using clinical protocols such as the Autism Observation Scale for Infants (AOSI) \textcolor{orange}{(What protocol did CFD use?)}
% Behavioral screening remains the gold standard for detecting, screening and assessing outcomes \hyeok{of what?} amongst individuals with ASD. However, clinical observation is often subjective, fails to study behaviors under natural environments and is not scalable to large populations or longitudinal studies \hyeok{because those screening assessments are clinician administered?}.
% \hyeok{This text is good. And it needs to be in the intro section! Also please put the citations ... any claim you make or any assessments you mention, NEED CITATIONS!}

 % \sout{Advanced technology \hyeok{Vague work, be more specific.} could play a key role in addressing these concerns and improving patient outcomes} \hyeok{of what?} \barun{removing this line as it doesn't add much}. There is a growing body of research geared towards behavioral imaging to quantify and understand behavioral signals outlined in various ASD protocols \hyeok{What protocols and what are specific examples?}.
% Hashemi et al. \hyeok{\textit{et al.} has to be italic} \cite{hashemi2015} created an app for autism screening by analyzing videos of toddlers aged 16-30 months as they watched developmentally appropriate visual stimuli \hyeok{what kind of visual stimuli?} on iPad.
% Specifically, they used a computer vision model to detect and classify facial expressions as positive, neutral or negative. \hyeok{why classifying emotions is important in ASD? And, you don't need to mentions computer vision every time. you can simply say that their method analyzed facial expression ... and so on.}
% They also performed social referencing \hyeok{what is this?} using head pose estimation from the collected video. 
% Their results demonstrate that automated analysis achieved good agreement \hyeok{what do you mean good? NEVER use such vague or qualitative word. how much was the agreement? do they report interrater reliability? or do they report any performance metric?} with human coding and computer coding for affect analysis and acceptable performance \hyeok{again what do you mean with acceptable performance?} for classification of social referencing.
% In another similar study, Bidwell et al. \cite{bidwell2014measuring} developed a markerless head tracking system using color and depth sensing cameras to study children's response to name by estimating head turn angles.
% The computer vision analysis was found to be comparable to a human analyst on reliability when predicting child response latency.
% Wang et al. \cite{wang2021rtn} proposed a vision system which achieved a mean classification score of 92.7\% in assistant screening of ASD \hyeok{what kind of study setting?}.
% These results demonstrate that computer vision tools are effective at capturing critical behavioral observations and automating analysis to detect ASD.

% Researchers have also studied other stereotyped behaviors in ASD, going beyond those described in protocols such as AOSI. 
% For instance, "stimming" refers to self-stimulatory behaviors involving repetitive, stereotyped movements of certain body parts, including  behaviors such as rocking, pacing and hand-flapping. 
% Rajagopalan proposed a computational model involving visual and speech signals to model common atypical behaviors in ASD such as stimming \cite{rgopalan2013stim}.
% They studied such behaviors in the context of a social dyadic conversational setting and validated their approach on human activity recognition datasets invloving repetitive behaviors as well as publicly available videos of children performing repetitive tasks
% There have also been works for automated analysis of autism behaviors.
% Vyas \textit{et al.} devised an algorithm to detect autistic characteristics from 2D poses in recorded videos of children \cite{vyas2019recognition}.
% Their work demonstrated a classification accuracy of 72\% when classifying typical and atypical behaviors on a target dataset containing 555 videos with a mix of both autistic behaviors and normal behaviors.
% Similarly, Scheithauer \textit{et al.} studied the feasibility of using accelerometers to monitor aggressive, self-injurious and disruptive behaviors in children with ASD during clinical assessments and in homes.


% \textcolor{orange}{\small \sout{(Most studies seem to focus on infants, while we have school-going children. Do autism behaviors differ among age groups? Can we point out some uniqueness given the age of the cohorts?)}}
% \hyeok{Which survey or review paper have you looked into?}
% \resolved


% However, previous work in this area has two major drawbacks: they either focused on curated datasets 
% \hyeok{it is not just a training dataset, right? they use their dataset for training and testing. So, you would just mention "dataset".}
% \resolved
% such as \cite{uci2017autismchildren} 
% \hyeok{just number cannot be citation. ALWAYS include author name} 
% \resolved
% which does not always replicate real-world conditions, such as during screening interviews, where patient behaviors are altered due to the setting \hyeok{I think "not always replicate real-world conditions" and "non-naturalistic settings" are same terms and no need to repeat.}.
% \hyeok{This drawback discussion in the previous work needs to be in introduction.}
% \resolved

% We address these concerns by teaming up with expert clinicians to study the natural behaviors of children with autism in a real-world classroom environment \hyeok{You main want to actually discuss what kind of classroom activities are conducted and what kind of problem behaviors are observed in our dataset.}. \hyeok{which work does not team up with developmental disorder experts? For ML specific work can be done by the engineering team, but still, the benchmark dataset is collected by someone working with specialists.}
% Additionally, we employed the attention mechanism to identify features with the most predictive power \hyeok{Most predictive power compared to what?}, thus improving the interpretability of model predictions \hyeok{what do you interpret? Be more specific.}.
% This helped our clinical partners evaluate the quality of predictions \hyeok{Is this really about the quality of predictions? Or is it about detecting novel features or objectively quantifying activity phenotypes in ASD that potentially will have high agreement with specialists?} made by the computer vision system compared to human analysts, thus validating our model predictions. 

% \hyeok{The related is shallow and needs better flow: 1) What are the kinds of problem behaviors in ASD from previous work? 2) What kind of approaches have been applied to quantify those behaviors before and currently with ML and which sensors and which settings? 3) What are the studies specifically used video-based approaches for ASD behavior analysis? Highlight our contribution in comparison to those previous work. What is our setting? 4) Previous work in applying explainable AI method and also examaples using Attention method? 5) explainable AI for health analytics and also specifically for ASD. 6) HIghlight our contribution of explainable AI in ASD behaviors 7) only briefly mention conclusion of our paper}
% \hyeok{Make sure you put CITATIONS for those additional discussions.}
% \hyeok{Try to merge these discussion with introduction appropriately.}

==> tables/frames-labeled.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{table}[H]
    \centering
    \begin{tabular}{ccc}
        % \hline
         \textbf{Camera} & \textbf{Frames} & \textbf{Videos} \\
         % \hline
         
         % \vspace{4pt}
        \small Cam 1 & \small 2,365,482 & \small 69 \\
        % \hline
         \small Cam 2 & \small 2,404,310 & \small 70 \\
    \end{tabular}
    \caption{\small Number of labeled videos and frames used in training for each camera in our study. \hyeok{Just say size of our dataset. And, use hours instead of frame numbers. But, do we really need a table that takes big space? I suggest removing this table and just mention those numbers in the main text where appropriate.}
    }
    \label{tab:frames}
\end{table}
